TextEssence: A Tool for Interactive Analysis of Semantic Shifts Between Corpora

Embeddings of words and concepts capture syntactic and semantic regularities of language; however, they have seen limited use as tools to study characteristics of different corpora and how they relate to one another. We introduce TextEssence, an interactive system designed to enable comparative analysis of corpora using embeddings. TextEssence includes visual, neighbor-based, and similarity-based modes of embedding analysis in a lightweight, web-based interface. We further propose a new measure of embedding confidence based on nearest neighborhood overlap, to assist in identifying high-quality embeddings for corpus analysis. A case study on COVID-19 scientific literature illustrates the utility of the system. TextEssence is available from https://github.com/drgriffis/text-essence.

==> figures/fig-confidence-distributions.tex <==
\begin{figure}
    \includegraphics[width=0.49\textwidth]{figures/images/confidence-distributions.png}
    \caption{Distributions of embedding confidence values (EC@5) for the eight
    months of CORD-19 analyzed. The high-confidence threshold of 0.5 is shown
    with a dashed line.}
    \label{fig:confidence-distributions}
\end{figure}

